GreaseLM: Graph REASoning Enhanced Language Models for Question Answering

Answering complex questions about textual narratives requires reasoning over both stated context and the world knowledge that underlies it. However, pretrained language models (LM), the foundation of most modern QA systems, do not robustly represent latent relationships between concepts, which is necessary for reasoning. While knowledge graphs (KG) are often used to augment LMs with structured representations of world knowledge, it remains an open question how to effectively fuse and reason over the KG representations and the language context, which provides situational constraints and nuances. In this work, we propose GreaseLM, a new model that fuses encoded representations from pretrained LMs and graph neural networks over multiple layers of modality interaction operations. Information from both modalities propagates to the other, allowing language context representations to be grounded by structured world knowledge, and allowing linguistic nuances (e.g., negation, hedging) in the context to inform the graph representations of knowledge. Our results on three benchmarks in the commonsense reasoning (i.e., CommonsenseQA, OpenbookQA) and medical question answering (i.e., MedQA-USMLE) domains demonstrate that GreaseLM can more reliably answer questions that require reasoning over both situational constraints and structured knowledge, even outperforming models 8x larger.

==> 4-model-old.tex <==


\section{Proposed Approach: \methodname}
\label{sec:model}

% \xikun{}
In this section, we present the overall framework of \methodname: the input representation in Section \ref{sec:model-input}, the model architecture in Section \ref{sec:model-arch}, the newly introduced \methodname layers in Section \ref{sec:model-layer}, and training and inference in Section \ref{sec:model-inference}.

\subsection{Notations}
We denote a sequence of tokens as $\tokens$, where $n$ is the total number of tokens, and the representation of a token $w_j$ in the $i$-th layer of the model as $\vh_{w_j}^{(i)}$. We denote a set of nodes as $\ents$, where $m$ is the total number of nodes, and the representation of a node $e_j$ in the $i$-th layer of the model as $\vg_{e_j}^{(i)}$.

\subsection{Input representation}
\label{sec:model-input}
Given an optional context paragraph $c$, a question $q$ and a candidate answer $a$, we concatenate them to get our QA context $[c;q;a]$. Then we do two preprocessing steps to construct the input so that it is ready to be fed into the model. First, we tokenize the QA context into a sequence of tokens $\tokens$. Second, we also use the QA context to retrieve a subgraph of the KG, which we denote as $\subgraph$, which is meant to provide the relevant information in the KG specific to this QA context. We denote the set of nodes in $\subgraph$ as $\ents$.

\paragraph{KG retrieval}
Given each QA context, in order to retrieve the subgraph $\subgraph$ from $\gG$, we follow the procedure used in \citet{Yasunaga2021QAGNNRW}. First, we perform entity linking to $\gG$ by which we can get an initial set of nodes $\gV$. Second, we add to $\gV$ any bridge entities that are in a 2-hop path between any pair of the linked entities. Third, we compute a relevance node score for each node in $\gV$ using a pretrained language model and use the node scores to prune the nodes using a preset threshold, forming the retrieved KG subgraph $\subgraph$. In the remaining parts of the paper, we use the term ``KG'' to refer to $\subgraph$.

\paragraph{Interaction token \& interaction node}
We also add one special token $t$ to the sequence of tokens and add one special node $z$ to the set of retrieved nodes, which we call \textit{interaction token} and \textit{interaction node} respectively. They serve as the "representatives" of the two modalities and directly interact in the model in a way which we will describe later. Specifically, we prepend $t$ to the token sequence and connect $z$ to all the \textit{linked} nodes in $\subgraph$, \ie the nodes retrieved in step 1 of the KG retrieval procedure.


\begin{figure}
    \centering
    \begin{minipage}{0.47\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/KaLM_Figure_v3.pdf}
        \caption{\methodname{} architecture with modality propagation layers at the top and bottom and interaction layers in the center}
        \label{fig:kalm1}
    \end{minipage}\hfill
    \begin{minipage}{0.47\textwidth}
        \centering
        \vspace{15pt}
        \includegraphics[width=\textwidth]{figures/KaLM_Figure_v2 2.pdf}
        % \vspace{1pt}
        \caption{Outline of \methodname's modality interaction layers. The MLP crosses each modality's representation.}
        \label{fig:kalm2}
    \end{minipage}
\end{figure}


\subsection{Model architecture}
\label{sec:model-arch}
As shown in Figure \ref{fig:kalm1}, \methodname consists of two stacked components: (1) the underlying uni-modal Tranformer LM layers which learn low-level lexical and syntactic information of the input tokens, and (2) the upper cross-modal \methodname layers which not only learn higher-level semantic information but also reason over the KG entities and relations and let textual representations from the underlying layers and the knowledge in KG deeply interact with each other. We denote the number of Transformer LM layers as $N$, and the number of \methodname layers as $M$.

Specifically, in the uni-modal encoding component, given the sequence of tokens $\{t, w_1, \dots, w_n\}$, we firstly sum the embedding, segment embedding, positional embedding for each token to compute its input embedding $\tokvec{0}$, and then computes lexical and syntactic features $\tokvec{i}$ in each layer as follows,

\begin{align}
    \tokvec{i} =& \text{ TransformerLM-Layer}(\tokvec{i - 1}) \nonumber \\
     &\text{ for } i = 1, \dots, N,
\end{align}
where TransformerLM-Layer($\cdot$) is a single Transformer encoder block, whose parameters we initialize using a pretrained RoBERTa LM. In terms of the technical details of these layers, we refer readers to \todocite{Transformers, Roberta}.

After computing $\tokvec{N}$ using the uni-modal encoding component, \methodname uses a cross-modal fusion component to inject the knowledge in the KG into the language representations. Specifically, we first compute the initial node embeddings $\{\ve_1^{(0)}, \dots, \ve_m^{(0)}\}$ by first using templates to turn knowledge triples in the KG into sentences, feeding them into a pretrained BERT-Large LM to get their embeddings and then performing mean pooling over the tokens of the entity’s occurrences across all the sentences, following \todocite{MHGRN}, finally followed by a linear transformation. The initial embedding of the interaction node $\vz^{0}$ is initialized randomly. Then both $\tokvec{N}$ and $\entvec{0}$ are fed into several \methodname layers for fusing the two modalities and computing the final output embeddings,

\begin{align}
    &\tokvec{N + i}, \entvec{i} \nonumber \\
    =& \text{ \methodname-Layer}(\tokvec{N + i - 1}, \entvec{i - 1}) \nonumber \\
     &\text{ for } i = 1, \dots, M.
\end{align}

The details of the \methodname-Layer($\cdot$) will be introduced in Section \ref{sec:model-layer}.
% Receiving this QA context and a KG $G$ available beforehand as input, \methodname output a probability score indicating the probability of the candidate answer $a$ being the correct answer of the question $a$ given the context $C$ and it works as follows. First, the QA context is passed to both a tokenizer, which outputs a list of tokens, and we also prepend a language interaction token $t$. We then pass this list of tokens through a language model, which is typically based on a multi-layer Transformer, which outputs a contextualized representation for each token. Second, the QA context is used to retrieve a subgraph of the KG, which we denote as $G_sub$. Then a multi-layer GNN takes in $G_sub$ 

\subsection{\methodname layer}
\label{sec:model-layer}

The \methodname layer is designed to both encode textual information and KG knowledge information as well as fusing the two modalities effectively. It is comprised of three components: (1) a Transformer-LM layer which learns language semantics, (2) a GNN layers that reason over KG entities and relations, and (3) a modality interaction layer that takes the representations from the above 2 components and exchanges information through the interaction token and the interaction node.

In the $i$-th \methodname layer, the input token embeddings $\tokvec{N + i - 1}$ are fed into a Transformer-LM layer, which outputs pre-fused token embeddings $\pftokvec{N + i}$,
\begin{align}
    \pftokvec{N + i} =& \text{ TransformerLM-Layer}(\tokvec{N + i - 1}).
\end{align}

\paragraph{GNN layer}
At the same time, the input node embeddings $\tokvec{i - 1}$ are fed into a GNN layer, which outputs pre-fused node embeddings $\pfentvec{N + i}$,
\begin{align}
    \pfentvec{i} =& \text{ GNN-Layer}(\entvec{i - 1}).
\end{align}

We adopt the same GNN architecture used in \citet{Yasunaga2021QAGNNRW}, which builds upon graph attention networks (GAT; \citealp{velickovic2018graph}). It induces node representations via message passing between neighbors on the graph. Specifically, we update the representation $\ve^{(i-1)}$ of each node $e \in \{e_1, \dots, e_m\}$ by

\begin{align}
    \tilde{\ve}^{(i)}= \text{ MLP}
    \Biggl(\sum_{s \in \mathcal{N}_{e} \cup \{e\} } \alpha_{se} \vm_{s e}\Biggr)
    +\ve^{(i-1)},
\end{align}

where $\gN_e$ represents the neighborhood of node $e$, $\vm_{s e}$ denotes the message its neighbor $s$ passes to $e$ and $\alpha_{se}$ is an attention weight that scales each message  $\vm_{s e}$. The sum of the messages across all its neighbors is passed through a 2-layer MLP. Crucially, message passing between the interaction node and the linked nodes enables exchanging information between the textual tokens and the KG nodes through a mechanism we will talk about below. The messages and the attention weights are calculated in a node type and relation-aware way. For the details of the computation of the messages and attention weights, we refer readers to \citet{Yasunaga2021QAGNNRW}.

\paragraph{Modality interaction layer}
Finally, after using a Transformer-LM layer and a GNN layer to update token embeddings and node embeddings respectively, we use a \textit{modality interaction layer} to let two modalities exchange information through the information bottleneck of the interaction token $t$ and the interaction node $z$. We concatenate the pre-fused embedding of the interaction token $\tilde{\vt}^{(i)}$ and that of the interaction node $\tilde{\vz}^{(i)}$, passed it through a 2-layer MLP, which outputs a vector with the same dimension as the input concatenated embedding, and then split it back into the post-fused embeddings of $\vt^{(i)}$ and $\vz^{(i)}$, 

\begin{align}
    [\vt^{(i)}; \vz^{(i)}] = \text{ MLP}([\tilde{\vt}^{(i)}; \tilde{\vz}^{(i)}]),
    \label{eq:interaction}
\end{align}

where $[;]$ means concatenation. All the tokens other than the interaction token $t$ and all the nodes other than the interaction node $z$ are not involved in the modality interaction process,

\begin{align}
    \vw^{(i)} &= \tilde{\vw}^{(i)} \text{ for } w \in \{w_1, \dots, w_n\} \\
    \ve^{(i)} &= \tilde{\ve}^{(i)} \text{ for } e \in \{e_1, \dots, e_m\}.
\end{align}


\subsection{Inference \& learning}
\label{sec:model-inference}
For the MCQA task, given a question $q$ and a candidate answer $a$ from all the candidates $C$, utilizing the information from both the QA context and the KG, we calculate the probability of $a$ being the answer as $p(a \mid q)\propto \exp(\text{MLP}(\vt^{(N+M)},~ \vz^{(M)},~ \vg))$, where $\vg$
denotes attention-based pooling of $\{\ve^{(M)} \mid e \in \{e_1, \dots, e_m\}\}$. 
In the training data, each question has a set of answer choices with one correct choice. We optimize the whole model end-to-end using the cross entropy loss. At inference time, we predict the most plausible answer as $\text{argmax}_{a \in C} ~ p(a \mid q)$.

% \paragraph{\methodname{} Nodes}

==> style/notation_reference.tex <==

\section{Default Notation}

In an attempt to encourage standardized notation, we have included the
notation file from the textbook, \textit{Deep Learning}
\cite{goodfellow2016deep} available at
\url{https://github.com/goodfeli/dlbook_notation/}.  Use of this style
is not required and can be disabled by commenting out
\texttt{math\_commands.tex}.


\centerline{\bf Numbers and Arrays}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1in}p{3.25in}}
$\displaystyle a$ & A scalar (integer or real)\\
$\displaystyle \va$ & A vector\\
$\displaystyle \mA$ & A matrix\\
$\displaystyle \tA$ & A tensor\\
$\displaystyle \mI_n$ & Identity matrix with $n$ rows and $n$ columns\\
$\displaystyle \mI$ & Identity matrix with dimensionality implied by context\\
$\displaystyle \ve^{(i)}$ & Standard basis vector $[0,\dots,0,1,0,\dots,0]$ with a 1 at position $i$\\
$\displaystyle \text{diag}(\va)$ & A square, diagonal matrix with diagonal entries given by $\va$\\
$\displaystyle \ra$ & A scalar random variable\\
$\displaystyle \rva$ & A vector-valued random variable\\
$\displaystyle \rmA$ & A matrix-valued random variable\\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Sets and Graphs}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \sA$ & A set\\
$\displaystyle \R$ & The set of real numbers \\
$\displaystyle \{0, 1\}$ & The set containing 0 and 1 \\
$\displaystyle \{0, 1, \dots, n \}$ & The set of all integers between $0$ and $n$\\
$\displaystyle [a, b]$ & The real interval including $a$ and $b$\\
$\displaystyle (a, b]$ & The real interval excluding $a$ but including $b$\\
$\displaystyle \sA \backslash \sB$ & Set subtraction, i.e., the set containing the elements of $\sA$ that are not in $\sB$\\
$\displaystyle \gG$ & A graph\\
$\displaystyle \parents_\gG(\ervx_i)$ & The parents of $\ervx_i$ in $\gG$
\end{tabular}
\vspace{0.25cm}


\centerline{\bf Indexing}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \eva_i$ & Element $i$ of vector $\va$, with indexing starting at 1 \\
$\displaystyle \eva_{-i}$ & All elements of vector $\va$ except for element $i$ \\
$\displaystyle \emA_{i,j}$ & Element $i, j$ of matrix $\mA$ \\
$\displaystyle \mA_{i, :}$ & Row $i$ of matrix $\mA$ \\
$\displaystyle \mA_{:, i}$ & Column $i$ of matrix $\mA$ \\
$\displaystyle \etA_{i, j, k}$ & Element $(i, j, k)$ of a 3-D tensor $\tA$\\
$\displaystyle \tA_{:, :, i}$ & 2-D slice of a 3-D tensor\\
$\displaystyle \erva_i$ & Element $i$ of the random vector $\rva$ \\
\end{tabular}
\egroup
\vspace{0.25cm}


\centerline{\bf Calculus}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
% NOTE: the [2ex] on the next line adds extra height to that row of the table.
% Without that command, the fraction on the first line is too tall and collides
% with the fraction on the second line.
$\displaystyle\frac{d y} {d x}$ & Derivative of $y$ with respect to $x$\\ [2ex]
$\displaystyle \frac{\partial y} {\partial x} $ & Partial derivative of $y$ with respect to $x$ \\
$\displaystyle \nabla_\vx y $ & Gradient of $y$ with respect to $\vx$ \\
$\displaystyle \nabla_\mX y $ & Matrix derivatives of $y$ with respect to $\mX$ \\
$\displaystyle \nabla_\tX y $ & Tensor containing derivatives of $y$ with respect to $\tX$ \\
$\displaystyle \frac{\partial f}{\partial \vx} $ & Jacobian matrix $\mJ \in \R^{m\times n}$ of $f: \R^n \rightarrow \R^m$\\
$\displaystyle \nabla_\vx^2 f(\vx)\text{ or }\mH( f)(\vx)$ & The Hessian matrix of $f$ at input point $\vx$\\
$\displaystyle \int f(\vx) d\vx $ & Definite integral over the entire domain of $\vx$ \\
$\displaystyle \int_\sS f(\vx) d\vx$ & Definite integral with respect to $\vx$ over the set $\sS$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Probability and Information Theory}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle P(\ra)$ & A probability distribution over a discrete variable\\
$\displaystyle p(\ra)$ & A probability distribution over a continuous variable, or over
a variable whose type has not been specified\\
$\displaystyle \ra \sim P$ & Random variable $\ra$ has distribution $P$\\% so thing on left of \sim should always be a random variable, with name beginning with \r
$\displaystyle  \E_{\rx\sim P} [ f(x) ]\text{ or } \E f(x)$ & Expectation of $f(x)$ with respect to $P(\rx)$ \\
$\displaystyle \Var(f(x)) $ &  Variance of $f(x)$ under $P(\rx)$ \\
$\displaystyle \Cov(f(x),g(x)) $ & Covariance of $f(x)$ and $g(x)$ under $P(\rx)$\\
$\displaystyle H(\rx) $ & Shannon entropy of the random variable $\rx$\\
$\displaystyle \KL ( P \Vert Q ) $ & Kullback-Leibler divergence of P and Q \\
$\displaystyle \mathcal{N} ( \vx ; \vmu , \mSigma)$ & Gaussian distribution %
over $\vx$ with mean $\vmu$ and covariance $\mSigma$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Functions}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle f: \sA \rightarrow \sB$ & The function $f$ with domain $\sA$ and range $\sB$\\
$\displaystyle f \circ g $ & Composition of the functions $f$ and $g$ \\
  $\displaystyle f(\vx ; \vtheta) $ & A function of $\vx$ parametrized by $\vtheta$.
  (Sometimes we write $f(\vx)$ and omit the argument $\vtheta$ to lighten notation) \\
$\displaystyle \log x$ & Natural logarithm of $x$ \\
$\displaystyle \sigma(x)$ & Logistic sigmoid, $\displaystyle \frac{1} {1 + \exp(-x)}$ \\
$\displaystyle \zeta(x)$ & Softplus, $\log(1 + \exp(x))$ \\
$\displaystyle || \vx ||_p $ & $\normlp$ norm of $\vx$ \\
$\displaystyle || \vx || $ & $\normltwo$ norm of $\vx$ \\
$\displaystyle x^+$ & Positive part of $x$, i.e., $\max(0,x)$\\
$\displaystyle \1_\mathrm{condition}$ & is 1 if the condition is true, 0 otherwise\\
\end{tabular}
\egroup
\vspace{0.25cm}

==> tables/tbl_csqa_leaderboard.tex <==
\begin{table}[tb]
\caption{\textbf{Test accuracy on \textit{CommonsenseQA}'s official leaderboard}. The top system, UnifiedQA (11B parameters) is 30x larger than our model.
}
% \vspace{-2mm}
\label{tab:csqa_leaderboard}
\centering
\small
% \scalebox{0.9}{
\begin{tabular}{lc}
\toprule
\textbf{Model}& \textbf{Test}  \\
\midrule
RoBERTa~\citep{liu2019roberta} & 72.1 \\

% \midrule
RoBERTa+FreeLB~\citep{zhu2019freelb} (ensemble) &73.1\\
RoBERTa+HyKAS~\citep{ma2019towards}&73.2\\
RoBERTa+KE (ensemble) & 73.3\\
RoBERTa+KEDGN (ensemble) & 74.4\\
XLNet+GraphReason~\citep{lv2020graph} & 75.3\\
RoBERTa+MHGRN \citep{feng2020scalable} & 75.4  \\
Albert+PG \citep{wang2020connecting} & 75.6  \\
% \midrule
Albert~\citep{lan2019albert} (ensemble) & 76.5 \\
UnifiedQA\textsuperscript{*}~\citep{khashabi2020unifiedqa} & \textbf{79.1} \\
\midrule
RoBERTa + (\textbf{Ours}) & 76.1 \\
\bottomrule
\end{tabular}
% }
\vspace{-2mm}
\end{table}



==> tables/tbl_medqa_main.tex <==
% \begin{table}[tb]
% \caption{\textbf{Test accuracy comparison on \textit{MedQA-USMLE}} (controlled experiments). }%\antoine{Add results from MedQA paper}}
% % \vspace{-2mm}
% \label{tab:medqa_main}
% % \hspace{-2mm}
% \centering
% % \scalebox{0.7}{
% \begin{tabular}{lc}
% \toprule
% \textbf{Methods}          & \textbf{Test Acc.} (\%)     \\
% \midrule
% \textbf{Baselines} \citep{jin2021disease} & \\
% \textsc{Chance}             & 25.0 \\ 
% \textsc{PMI}                & 31.1 \\ 
% \textsc{IR-ES}              & 35.5 \\ 
% \textsc{IR-Custom}          & 36.1 \\ 
% \textsc{Max-out}            & 28.6 \\ 
% \textsc{BERT-Base-En}       & 34.3 \\ 
% \textsc{clinicalBERT-Base}  & 32.4 \\ 
% \textsc{BioRoBERTa-Base}    & 36.1 \\ 
% \textsc{BioBERT-Base}       & 34.1 \\ 
% \textsc{RoBERTa-Large}      & 35.0 \\ 
% \textsc{BioBERT-Large}      & 36.7 \\
% \midrule
% \textbf{Baselines} (Ours) & \\
% SapBERT-Base (w/o KG)          & 37.2     \\
% % \midrule
% % + RGCN           & 74.60~($\pm$2.53)
% %       \\
% % + GconAtten      & 71.80~($\pm$1.21)
% %       \\
% % + RN             & 75.35~($\pm$1.39)
% %       \\
% % + MHGRN  & 80.6        \\
% + QA-GNN       &  38.0  \\
% \midrule
% + \methodname (\textbf{Ours})  &  \textbf{38.4}   \\

% \bottomrule
% \end{tabular}
% % }
% \vspace{-2mm}
% \end{table}


==> tables/tbl_obqa_leaderboard.tex <==
\begin{table}[h]
\caption{\textbf{Test accuracy on \textit{OpenBookQA} leaderboard}. All listed methods use the provided scientific facts as an additional input along with the language context. UnifiedQA (11B params) and T5 (3B params) are 30x and 8x larger than our model respectively.}
% \vspace{-2mm}
\label{tab:obqa_leaderboard}
\centering
% \small
% \scalebox{0.9}{
\begin{tabular}{lc}
\toprule
\textbf{Model}         & \textbf{Test}           \\
\midrule
ALBERT \citep{lan2019albert} + KB & 81.0\\
AristoRoBERTa + HGN \citep{yan2020learning} & 81.4 \\
AristoRoBERTa + AMR-SG \citep{xu2021dynamic} & 81.6 \\
ALBERT + KPG \citep{wang2020connecting} & 81.8 \\
AristoRoBERTa + CGR & 82.4 \\
AristoRoBERTa + QAGNN \citep{Yasunaga2021QAGNNRW}  & 82.8\\
T5\textsuperscript{*}~\citep{t5} & 83.2\\
T5 + KB & 85.4\\
UnifiedQA\textsuperscript{*}~\citep{khashabi2020unifiedqa} &$\textbf{87.2}$          \\
\midrule
AristoRoBERTa + \methodname (\textbf{Ours}) & 84.6\\
\bottomrule
\end{tabular}
% }
\vspace{-2mm}
\end{table}

==> tables/tbl_obqa_main.tex <==
\begin{table}[tb]
\caption{\textbf{Test accuracy comparison on \textit{OpenBook \!\!QA}} (controlled experiments). All methods here use the textual facts prepared by \citet{clark2019f} as an additional input along with the QA context.}
% \vspace{-2mm}
\label{tab:obqa_main}
% \hspace{-2mm}
\centering
% \scalebox{0.7}{
\begin{tabular}{lc}
\toprule
\textbf{Model}          & \textbf{Test Acc.} (\%)     \\
\midrule
AristoRoBERTa (no KG)          & 78.40~($\pm$1.64)       \\
\midrule
+ RGCN           & 74.60~($\pm$2.53)
       \\
+ GconAtten      & 71.80~($\pm$1.21)
       \\
+ RN             & 75.35~($\pm$1.39)
       \\
+ MHGRN  & 80.6        \\
+ QA-GNN       &  82.77~($\pm$1.56)    \\
\midrule
+ \methodname (\textbf{Ours})       &  \textbf{84.6}    \\

\bottomrule
\end{tabular}
% }
\vspace{-2mm}
\end{table}


==> tables/tbl_socialiqa_main.tex <==
\begin{table}[tb]
\caption{\textbf{Dev accuracy comparison on \textit{SocialIQA}} (controlled experiments).}
% \vspace{-2mm}
\label{tab:socialiqa_main}
% \hspace{-2mm}
\centering
% \scalebox{0.7}{
\begin{tabular}{lc}
\toprule
\textbf{Methods}          & \textbf{Dev Acc.} (\%)     \\
\midrule
RoBERTa-large (w/o KG)          & 78.3     \\
\midrule
% + RGCN           & 74.60~($\pm$2.53)
%       \\
% + GconAtten      & 71.80~($\pm$1.21)
%       \\
% + RN             & 75.35~($\pm$1.39)
%       \\
% + MHGRN  & 80.6        \\
% + QA-GNN       &  82.77~($\pm$1.56)    \\
\midrule
+ \methodname (\textbf{Ours})       &  78.6   \\

\bottomrule
\end{tabular}
% }
\vspace{-2mm}
\end{table}

